Privacy-preserving Reflection Rendering for Augmented Reality

Many augmented reality (AR) applications rely on omnidirectional environment lighting to render photorealistic virtual objects. When the virtual objects consist of reflective materials, such as a metallic sphere, the required lighting information to render such objects can consist of privacy-sensitive information that is outside the current camera view. In this paper, we show, for the first time, that accuracy-driven multi-view environment lighting can reveal out-of-camera scene information and compromise privacy. We present a simple yet effective privacy attack that extracts sensitive scene information such as human face and text information from the rendered objects, under a number of application scenarios. To defend against such attacks, we develop a novel $IPC^{2}S$ defense and a conditional $R^2$ defense. Our $IPC^{2}S$ defense, used in conjunction with a generic lighting reconstruction method, preserves the scene geometry while obfuscating the privacy-sensitive information. As a proof-of-concept, we leverage existing OCR and face detection models to identify text and human faces from past camera observations and blur the color pixels associated with detected regions. We evaluate the visual quality impact of our defense by comparing rendered virtual objects to ones rendered with a generic multi-lighting reconstruction technique, ARKit, and $R^2$ defense. Our visual and quantitative results demonstrate that our defense leads to structurally similar reflections with up to 0.98 SSIM score across a variety of rendering scenarios while preserving sensitive information by reducing the automatic extraction success rate to at most 8.8%.

==> Privacy_Preserving_Reflection_arXiv'22/results/fig_attack_illustration.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.9\textwidth]{img/attack_visualization.pdf}
    \caption{The reflection-based privacy issues in AR content creation and streaming.
    \textnormal{We demonstrate the general workflow of AR streaming to highlight how the rendered reflection of virtual sunglasses can contain sensitive information from the streamer Alice's physical surroundings and be leaked to the viewer Malice.
    }
    }
    \label{fig:AR_streaming_workflow}
    \vspace{-4mm}
\end{figure*}


==> Privacy_Preserving_Reflection_arXiv'22/results/fig_defenes_procedure.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.9\textwidth]{img/defense_pipeline.pdf}
    \caption{
    Our proposed defense for preserving reflection-based privacy for AR streaming. 
    \textnormal{Our defense pipeline is designed around the key idea of index-based point color swapping to obfuscate the visual detail of the sensitive information while still maintaining the overall reflection color pattern.
    Moreover, the defense pipeline can run in parallel to the generic lighting reconstruction pipeline described in Sec~\ref{sec:lighting_reconstruction_premier}.
    }
    }
    \label{fig:reflection_extraction}
    \vspace{-3mm}
\end{figure*}


==> Privacy_Preserving_Reflection_arXiv'22/results/fig_defense_visual_impacts.tex <==
\begin{figure}[t]
    \centering
    % \includegraphics[width=3.4in]{img/placeholder.pdf}
    % \caption{
    %     Defense effectiveness. \yiqin{TODO: adding results about defense success/failure rate, } 
    % }
    % \label{fig:defense_effectiveness}
    
    \begin{subfigure}[b]{0.45\linewidth}
        \centering
        % \includegraphics[width=\linewidth]{assets/xihenet_shc_rmse.pdf}
        \includegraphics[width=\linewidth]{img/pair_wise_psnr.pdf}
        \vspace{-5mm}
        \caption{Rendering PSNR.
        % \tian{why test error increases for larger anchor size?}
        % \tian{TODO: can add a new line to represent the non-accelerated inference (edge)!}
        }
        \label{subfig:psnr}
    \end{subfigure}%
    \quad
    \begin{subfigure}[b]{0.45\linewidth}
        \centering
        % \includegraphics[width=\linewidth]{assets/triton_throughput.pdf}
        \includegraphics[width=\linewidth]{img/pair_wise_ssim.pdf}
        \vspace{-5mm}
        \caption{Rendering SSIM
        % \tian{anything else that will impact the throughput besides the anchor size?}
        }
        \label{subfig:ssim}
    \end{subfigure}
    
    % \begin{subfigure}[b]{0.45\linewidth}
    %     \centering
    %     % \includegraphics[width=\linewidth]{assets/xihenet_shc_rmse.pdf}
    %     \includegraphics[width=\linewidth]{img/pair_wise_psnr_ball.pdf}
    %     \caption{Metal Ball Rendering PSNR.
    %     % \tian{why test error increases for larger anchor size?}
    %     % \tian{TODO: can add a new line to represent the non-accelerated inference (edge)!}
    %     }
    %     \label{subfig:ball_psnr}
    % \end{subfigure}%
    % \quad
    % \begin{subfigure}[b]{0.45\linewidth}
    %     \centering
    %     % \includegraphics[width=\linewidth]{assets/triton_throughput.pdf}
    %     \includegraphics[width=\linewidth]{img/pair_wise_psnr_mirror.pdf}
    %     \caption{Mirror Rendering PSNR
    %     % \tian{anything else that will impact the throughput besides the anchor size?}
    %     }
    %     \label{subfig:mirror_psnr}
    % \end{subfigure}
    
    % \begin{subfigure}[b]{0.45\linewidth}
    %     \centering
    %     % \includegraphics[width=\linewidth]{assets/xihenet_shc_rmse.pdf}
    %     \includegraphics[width=\linewidth]{img/pair_wise_ssim_ball.pdf}
    %     \caption{Metal Ball Rendering SSIM.
    %     % \tian{why test error increases for larger anchor size?}
    %     % \tian{TODO: can add a new line to represent the non-accelerated inference (edge)!}
    %     }
    %     \label{subfig:ball_ssim}
    % \end{subfigure}%
    % \quad
    % \begin{subfigure}[b]{0.45\linewidth}
    %     \centering
    %     % \includegraphics[width=\linewidth]{assets/triton_throughput.pdf}
    %     \includegraphics[width=\linewidth]{img/pair_wise_ssim_mirror.pdf}
    %     \caption{Mirror Rendering SSIM
    %     % \tian{anything else that will impact the throughput besides the anchor size?}
    %     }
    %     \label{subfig:mirrow_ssim}
    % \end{subfigure}
    
     \vspace{-4mm}
    
    \caption{
        Quantitative comparisons of our \defense and \renderingdefense.
        \textnormal{
        \defense achieves high PSNR and SSIM scores while \renderingdefense has at least 0.91 and 0.82 SSIM values. 
        }
    }
    \label{fig:defense_visual_impacts}
    \vspace{-3mm}
\end{figure}


==> Privacy_Preserving_Reflection_arXiv'22/results/fig_renderings.tex <==
\begin{figure*}[t]
    \centering
    % \includegraphics[width=3.2in]{img/volumetric_video_streaming_arch.png}
    \includegraphics[width=\textwidth]{img/vis_rendering.pdf} % width=3.2in
    \caption{
    %\tian{A}
        Reflection renderings..
        % \yiqin{TODO: replace with more realistic objects rendering}
        \yiqin{
            TODO: Add zoomed thumbnails, Bug: row marks, also make the texts bigger maybe.
            To be discussed: break this figure into two figures, one for showing renderings on ball and mirror. And another one for comparing raw, restricted and def.
        }
    }
    \label{fig:renderings}
\end{figure*}


==> Privacy_Preserving_Reflection_arXiv'22/results/fig_vis_attack.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{img/fig_vis_attack.pdf} % width=3.2in
    \vspace{-5mm}
    \caption{
        The visual effectiveness of our attack on reflection-based privacy.
        \textnormal{
        Row one shows the reflection rendering of two virtual objects;
        row two zooms in on the four types of sensitive information leakage.
        }
    }
    \label{fig:vis_attack}
    \vspace{-3mm}
\end{figure*}


==> Privacy_Preserving_Reflection_arXiv'22/results/fig_vis_defense_visuals.tex <==
\begin{figure}[t]
    \centering
    % \includegraphics[width=3.2in]{img/volumetric_video_streaming_arch.png}
    \includegraphics[width=\linewidth]{img/vis_defenes_visuals.pdf} % width=3.2in
    \vspace{-5mm}
    \caption{
        The low visual impact of our defense on reflection-based privacy.
        \textnormal{
        \defense achieves similar reflective visual quality compared to a re-implemented pipeline~\cite{zhao2022FusedAR}. 
        }
    }
    \label{fig:vis_defense_visuals}
    % \vspace{-6mm}
\end{figure}


==> Privacy_Preserving_Reflection_arXiv'22/results/tab_attack_results.tex <==
\setlength{\tabcolsep}{3pt}
\begin{table}[t]
\centering
% \vspace{-0.5em}
\caption{The high success rate of our attack.
\textnormal{On average we can manually extract 100\% human face information and at least 92\% textual information.
The automatic extraction has lower success rates but still poses considerable privacy issues.
}
}
\vspace{-2mm}
\small{ % scriptsize
\begin{tabular}{lrrrrr}
\toprule
% 
% \begin{tabular}[r]{@{}r@{}}\textbf{Sensitive}\\ \textbf{Info.}\end{tabular} \\
% & \begin{tabular}[r]{@{}r@{}}\textbf{Virtual}\\ \textbf{Object}\end{tabular} \\
\textbf{Sensitive} & \textbf{Virtual} & \multicolumn{2}{r}{\textbf{Face Recognition}} & \multicolumn{2}{r}{\textbf{Text Recognition}} \\ 
\textbf{Info} & \textbf{Object} & \textbf{\textit{Automatic}} & \textbf{\textit{Manual}} & \textbf{\textit{Automatic}} & \textbf{\textit{Manual}}\\
% & \begin{tabular}[r]{@{}r@{}}\textbf{Automatic}\\ \textbf{Human}\end{tabular}
% & \begin{tabular}[r]{@{}r@{}}\textbf{Text}\\ \textbf{Recognition}\end{tabular}\\

\midrule

Driver's                & Metal Ball    & 50.00\%  & 100.00\% & 33.33\% & 87.50\% \\
% \cdashline{2-6} License 1   & Mirror        & 100.00\% & 100.00\% & 81.94\% & 97.83\% \\
License 1   & Mirror        & 100.00\% & 100.00\% & 81.94\% & 97.83\% \\

\midrule

Driver's                & Metal Ball    & 100.00\% & 100.00\% & 20.59\% & 94.12\% \\
% \cdashline{2-6} License 2   & Mirror        & 100.00\% & 100.00\% & 80.88\% & 95.59\% \\
License 2   & Mirror        & 100.00\% & 100.00\% & 80.88\% & 95.59\% \\

\midrule

Group                   & Metal Ball    & 17.85\%  & 100.00\% & N/A & N/A \\
% \cdashline{2-6} Photo       & Mirror        & 96.42\%  & 100.00\% & N/A & N/A \\
Photo       & Mirror        & 96.42\%  & 100.00\% & N/A & N/A \\

\midrule

Credit                  & Metal Ball    & N/A    & N/A & 75.00\% & 96.42\% \\
% \cdashline{2-6} Card        & Mirror        & N/A    & N/A & 71.42\% & 96.42\% \\
Card        & Mirror        & N/A    & N/A & 71.42\% & 96.42\% \\

\midrule

\emph{Average}                 & Metal Ball    & 29.41\%      & 100.00\%  & 35.11\% & 91.67\% \\
% \cdashline{2-6} Average & Mirror        & 97.06\%      & 100.00\%  & 79.76\% & 95.83\% \\
\emph{Average} & Mirror        & 97.06\%      & 100.00\%  & 79.76\% & 95.83\% \\

\bottomrule

\end{tabular}
}
\label{tab:attack_results}
\vspace{-5mm}
\end{table}


==> Privacy_Preserving_Reflection_arXiv'22/results/tab_defense_results.tex <==
\setlength{\tabcolsep}{3pt}
\begin{table}[t]
\centering
% \vspace{-0.5em}
\caption{
The low success rate when using our \defense.
\textnormal{
On average, this defense effectively decreases the success rate of automatic extraction to at most 8.8\%/5.4\% and manual extraction to at most 11.8\%/23.8\% for face/text information. 
}
}
\vspace{-3mm}
\small{ % scriptsize
\begin{tabular}{lrrrrr}
\toprule
% 
\textbf{Sensitive} & \textbf{Virtual} & \multicolumn{2}{r}{\textbf{Face Recognition}} & \multicolumn{2}{r}{\textbf{Text Recognition}} \\
\textbf{Info} & \textbf{Object} & \textbf{\textit{Automatic}} & \textbf{\textit{Manual}} & \textbf{\textit{Automatic}} & \textbf{\textit{Manual}}\\

\midrule

Driver's                    & Metal Ball    & 0.00\% & 0.00\% & 0.00\% & 16.67\% \\
%\cdashline{2-6} License 1   & Mirror        & 0.00\% & 0.00\% & 6.94\% & 18.06\% \\
License 1                   & Mirror        & 0.00\% & 0.00\% & 6.94\% & 18.06\% \\

\midrule

Driver's                    & Metal Ball    & 0.00\% & 0.00\% & 0.00\% & 30.88\% \\
% \cdashline{2-6} License 2   & Mirror        & 0.00\% & 0.00\% & 5.88\% & 36.76\% \\
License 2   & Mirror        & 0.00\% & 0.00\% & 5.88\% & 36.76\% \\

\midrule

Group                       & Metal Ball    & 0.00\%     & 14.29\% & N/A & N/A \\
% \cdashline{2-6} Photo       & Mirror        & 10.71\%    & 14.29\% & N/A & N/A \\
Photo       & Mirror        & 10.71\%    & 14.29\% & N/A & N/A \\

\midrule

Credit                      & Metal Ball    & N/A    & N/A & 0.00\% & 3.57\% \\
% \cdashline{2-6} Card        & Mirror        & N/A    & N/A & 0.00\% & 7.14\% \\
Card        & Mirror        & N/A    & N/A & 0.00\% & 7.14\% \\

\midrule

\emph{Average}                     & Metal Ball    & 0.00\%     & 11.76\%  & 0.00\% & 20.24\% \\
% \cdashline{2-6} Average     & Mirror        & 8.82\%     & 11.76\%  & 5.36\% & 23.81\% \\
\emph{Average}     & Mirror        & 8.82\%     & 11.76\%  & 5.36\% & 23.81\% \\

\bottomrule

\end{tabular}
}
\label{tab:defense_results}
\vspace{-2mm}
\end{table}



==> results/fig_attack_illustration.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.9\textwidth]{img/attack_visualization.pdf}
    \caption{The reflection-based privacy issues in AR content creation and streaming.
    \textnormal{We demonstrate the general workflow of AR streaming to highlight how the rendered reflection of virtual sunglasses can contain sensitive information from the streamer Alice's physical surroundings and be leaked to the viewer Malice.
    }
    }
    \label{fig:AR_streaming_workflow}
    \vspace{-4mm}
\end{figure*}


==> results/fig_defenes_procedure.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.9\textwidth]{img/defense_pipeline.pdf}
    \caption{
    Our proposed defense for preserving reflection-based privacy for AR streaming. 
    \textnormal{Our defense pipeline is designed around the key idea of index-based point color swapping to obfuscate the visual detail of the sensitive information while still maintaining the overall reflection color pattern.
    Moreover, the defense pipeline can run in parallel to the generic lighting reconstruction pipeline described in Sec~\ref{sec:lighting_reconstruction_premier}.
    }
    }
    \label{fig:reflection_extraction}
    \vspace{-3mm}
\end{figure*}


==> results/fig_defense_visual_impacts.tex <==
\begin{figure}[t]
    \centering
    % \includegraphics[width=3.4in]{img/placeholder.pdf}
    % \caption{
    %     Defense effectiveness. \yiqin{TODO: adding results about defense success/failure rate, } 
    % }
    % \label{fig:defense_effectiveness}
    
    \begin{subfigure}[b]{0.45\linewidth}
        \centering
        % \includegraphics[width=\linewidth]{assets/xihenet_shc_rmse.pdf}
        \includegraphics[width=\linewidth]{img/pair_wise_psnr.pdf}
        \vspace{-5mm}
        \caption{Rendering PSNR.
        % \tian{why test error increases for larger anchor size?}
        % \tian{TODO: can add a new line to represent the non-accelerated inference (edge)!}
        }
        \label{subfig:psnr}
    \end{subfigure}%
    \quad
    \begin{subfigure}[b]{0.45\linewidth}
        \centering
        % \includegraphics[width=\linewidth]{assets/triton_throughput.pdf}
        \includegraphics[width=\linewidth]{img/pair_wise_ssim.pdf}
        \vspace{-5mm}
        \caption{Rendering SSIM
        % \tian{anything else that will impact the throughput besides the anchor size?}
        }
        \label{subfig:ssim}
    \end{subfigure}
    
    % \begin{subfigure}[b]{0.45\linewidth}
    %     \centering
    %     % \includegraphics[width=\linewidth]{assets/xihenet_shc_rmse.pdf}
    %     \includegraphics[width=\linewidth]{img/pair_wise_psnr_ball.pdf}
    %     \caption{Metal Ball Rendering PSNR.
    %     % \tian{why test error increases for larger anchor size?}
    %     % \tian{TODO: can add a new line to represent the non-accelerated inference (edge)!}
    %     }
    %     \label{subfig:ball_psnr}
    % \end{subfigure}%
    % \quad
    % \begin{subfigure}[b]{0.45\linewidth}
    %     \centering
    %     % \includegraphics[width=\linewidth]{assets/triton_throughput.pdf}
    %     \includegraphics[width=\linewidth]{img/pair_wise_psnr_mirror.pdf}
    %     \caption{Mirror Rendering PSNR
    %     % \tian{anything else that will impact the throughput besides the anchor size?}
    %     }
    %     \label{subfig:mirror_psnr}
    % \end{subfigure}
    
    % \begin{subfigure}[b]{0.45\linewidth}
    %     \centering
    %     % \includegraphics[width=\linewidth]{assets/xihenet_shc_rmse.pdf}
    %     \includegraphics[width=\linewidth]{img/pair_wise_ssim_ball.pdf}
    %     \caption{Metal Ball Rendering SSIM.
    %     % \tian{why test error increases for larger anchor size?}
    %     % \tian{TODO: can add a new line to represent the non-accelerated inference (edge)!}
    %     }
    %     \label{subfig:ball_ssim}
    % \end{subfigure}%
    % \quad
    % \begin{subfigure}[b]{0.45\linewidth}
    %     \centering
    %     % \includegraphics[width=\linewidth]{assets/triton_throughput.pdf}
    %     \includegraphics[width=\linewidth]{img/pair_wise_ssim_mirror.pdf}
    %     \caption{Mirror Rendering SSIM
    %     % \tian{anything else that will impact the throughput besides the anchor size?}
    %     }
    %     \label{subfig:mirrow_ssim}
    % \end{subfigure}
    
     \vspace{-4mm}
    
    \caption{
        Quantitative comparisons of our \defense and \renderingdefense.
        \textnormal{
        \defense achieves high PSNR and SSIM scores while \renderingdefense has at least 0.91 and 0.82 SSIM values. 
        }
    }
    \label{fig:defense_visual_impacts}
    \vspace{-3mm}
\end{figure}


==> results/fig_renderings.tex <==
\begin{figure*}[t]
    \centering
    % \includegraphics[width=3.2in]{img/volumetric_video_streaming_arch.png}
    \includegraphics[width=\textwidth]{img/vis_rendering.pdf} % width=3.2in
    \caption{
    %\tian{A}
        Reflection renderings..
        % \yiqin{TODO: replace with more realistic objects rendering}
        \yiqin{
            TODO: Add zoomed thumbnails, Bug: row marks, also make the texts bigger maybe.
            To be discussed: break this figure into two figures, one for showing renderings on ball and mirror. And another one for comparing raw, restricted and def.
        }
    }
    \label{fig:renderings}
\end{figure*}


==> results/fig_vis_attack.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{img/fig_vis_attack.pdf} % width=3.2in
    \vspace{-5mm}
    \caption{
        The visual effectiveness of our attack on reflection-based privacy.
        \textnormal{
        Row one shows the reflection rendering of two virtual objects;
        row two zooms in on the four types of sensitive information leakage.
        }
    }
    \label{fig:vis_attack}
    \vspace{-3mm}
\end{figure*}


==> results/fig_vis_defense_visuals.tex <==
\begin{figure}[t]
    \centering
    % \includegraphics[width=3.2in]{img/volumetric_video_streaming_arch.png}
    \includegraphics[width=\linewidth]{img/vis_defenes_visuals.pdf} % width=3.2in
    \vspace{-5mm}
    \caption{
        The low visual impact of our defense on reflection-based privacy.
        \textnormal{
        \defense achieves similar reflective visual quality compared to a re-implemented pipeline~\cite{zhao2022FusedAR}. 
        }
    }
    \label{fig:vis_defense_visuals}
    % \vspace{-6mm}
\end{figure}


==> results/tab_attack_results.tex <==
\setlength{\tabcolsep}{3pt}
\begin{table}[t]
\centering
% \vspace{-0.5em}
\caption{The high success rate of our attack.
\textnormal{On average we can manually extract 100\% human face information and at least 92\% textual information.
The automatic extraction has lower success rates but still poses considerable privacy issues.
}
}
\vspace{-2mm}
\small{ % scriptsize
\begin{tabular}{lrrrrr}
\toprule
% 
% \begin{tabular}[r]{@{}r@{}}\textbf{Sensitive}\\ \textbf{Info.}\end{tabular} \\
% & \begin{tabular}[r]{@{}r@{}}\textbf{Virtual}\\ \textbf{Object}\end{tabular} \\
\textbf{Sensitive} & \textbf{Virtual} & \multicolumn{2}{r}{\textbf{Face Recognition}} & \multicolumn{2}{r}{\textbf{Text Recognition}} \\ 
\textbf{Info} & \textbf{Object} & \textbf{\textit{Automatic}} & \textbf{\textit{Manual}} & \textbf{\textit{Automatic}} & \textbf{\textit{Manual}}\\
% & \begin{tabular}[r]{@{}r@{}}\textbf{Automatic}\\ \textbf{Human}\end{tabular}
% & \begin{tabular}[r]{@{}r@{}}\textbf{Text}\\ \textbf{Recognition}\end{tabular}\\

\midrule

Driver's                & Metal Ball    & 50.00\%  & 100.00\% & 33.33\% & 87.50\% \\
% \cdashline{2-6} License 1   & Mirror        & 100.00\% & 100.00\% & 81.94\% & 97.83\% \\
License 1   & Mirror        & 100.00\% & 100.00\% & 81.94\% & 97.83\% \\

\midrule

Driver's                & Metal Ball    & 100.00\% & 100.00\% & 20.59\% & 94.12\% \\
% \cdashline{2-6} License 2   & Mirror        & 100.00\% & 100.00\% & 80.88\% & 95.59\% \\
License 2   & Mirror        & 100.00\% & 100.00\% & 80.88\% & 95.59\% \\

\midrule

Group                   & Metal Ball    & 17.85\%  & 100.00\% & N/A & N/A \\
% \cdashline{2-6} Photo       & Mirror        & 96.42\%  & 100.00\% & N/A & N/A \\
Photo       & Mirror        & 96.42\%  & 100.00\% & N/A & N/A \\

\midrule

Credit                  & Metal Ball    & N/A    & N/A & 75.00\% & 96.42\% \\
% \cdashline{2-6} Card        & Mirror        & N/A    & N/A & 71.42\% & 96.42\% \\
Card        & Mirror        & N/A    & N/A & 71.42\% & 96.42\% \\

\midrule

\emph{Average}                 & Metal Ball    & 29.41\%      & 100.00\%  & 35.11\% & 91.67\% \\
% \cdashline{2-6} Average & Mirror        & 97.06\%      & 100.00\%  & 79.76\% & 95.83\% \\
\emph{Average} & Mirror        & 97.06\%      & 100.00\%  & 79.76\% & 95.83\% \\

\bottomrule

\end{tabular}
}
\label{tab:attack_results}
\vspace{-5mm}
\end{table}


==> results/tab_defense_results.tex <==
\setlength{\tabcolsep}{3pt}
\begin{table}[t]
\centering
% \vspace{-0.5em}
\caption{
The low success rate when using our \defense.
\textnormal{
On average, this defense effectively decreases the success rate of automatic extraction to at most 8.8\%/5.4\% and manual extraction to at most 11.8\%/23.8\% for face/text information. 
}
}
\vspace{-3mm}
\small{ % scriptsize
\begin{tabular}{lrrrrr}
\toprule
% 
\textbf{Sensitive} & \textbf{Virtual} & \multicolumn{2}{r}{\textbf{Face Recognition}} & \multicolumn{2}{r}{\textbf{Text Recognition}} \\
\textbf{Info} & \textbf{Object} & \textbf{\textit{Automatic}} & \textbf{\textit{Manual}} & \textbf{\textit{Automatic}} & \textbf{\textit{Manual}}\\

\midrule

Driver's                    & Metal Ball    & 0.00\% & 0.00\% & 0.00\% & 16.67\% \\
%\cdashline{2-6} License 1   & Mirror        & 0.00\% & 0.00\% & 6.94\% & 18.06\% \\
License 1                   & Mirror        & 0.00\% & 0.00\% & 6.94\% & 18.06\% \\

\midrule

Driver's                    & Metal Ball    & 0.00\% & 0.00\% & 0.00\% & 30.88\% \\
% \cdashline{2-6} License 2   & Mirror        & 0.00\% & 0.00\% & 5.88\% & 36.76\% \\
License 2   & Mirror        & 0.00\% & 0.00\% & 5.88\% & 36.76\% \\

\midrule

Group                       & Metal Ball    & 0.00\%     & 14.29\% & N/A & N/A \\
% \cdashline{2-6} Photo       & Mirror        & 10.71\%    & 14.29\% & N/A & N/A \\
Photo       & Mirror        & 10.71\%    & 14.29\% & N/A & N/A \\

\midrule

Credit                      & Metal Ball    & N/A    & N/A & 0.00\% & 3.57\% \\
% \cdashline{2-6} Card        & Mirror        & N/A    & N/A & 0.00\% & 7.14\% \\
Card        & Mirror        & N/A    & N/A & 0.00\% & 7.14\% \\

\midrule

\emph{Average}                     & Metal Ball    & 0.00\%     & 11.76\%  & 0.00\% & 20.24\% \\
% \cdashline{2-6} Average     & Mirror        & 8.82\%     & 11.76\%  & 5.36\% & 23.81\% \\
\emph{Average}     & Mirror        & 8.82\%     & 11.76\%  & 5.36\% & 23.81\% \\

\bottomrule

\end{tabular}
}
\label{tab:defense_results}
\vspace{-2mm}
\end{table}


